MegaPose: 6D Pose Estimation of Novel Objects via Render & Compare

We introduce MegaPose, a method to estimate the 6D pose of novel objects, that is, objects unseen during training. At inference time, the method only assumes knowledge of (i) a region of interest displaying the object in the image and (ii) a CAD model of the observed object. The contributions of this work are threefold. First, we present a 6D pose refiner based on a render&compare strategy which can be applied to novel objects. The shape and coordinate system of the novel object are provided as inputs to the network by rendering multiple synthetic views of the object's CAD model. Second, we introduce a novel approach for coarse pose estimation which leverages a network trained to classify whether the pose error between a synthetic rendering and an observed image of the same object can be corrected by the refiner. Third, we introduce a large-scale synthetic dataset of photorealistic images of thousands of objects with diverse visual and shape properties and show that this diversity is crucial to obtain good generalization performance on novel objects. We train our approach on this large synthetic dataset and apply it without retraining to hundreds of novel objects in real images from several pose estimation benchmarks. Our approach achieves state-of-the-art performance on the ModelNet and YCB-Video datasets. An extensive evaluation on the 7 core datasets of the BOP challenge demonstrates that our approach achieves performance competitive with existing approaches that require access to the target objects during training. Code, dataset and trained models are available on the project page: https://megapose6d.github.io/.

==> deprecated.tex <==
{
\color{red}

\section{Method}
\label{sec:approach}

In this section we present our framework for pose estimation of novel objects. 
Our goal is to detect the pose $\tT_{\textit{CO}}$\footnote{$\TCO$ denotes the object pose expressed in camera frame} of a novel object given an input RGB (or RGBD) image, $I_o$, and a 3D model of the object. 
Similar to DeepIM \citep{li2018deepim} and CosyPose \citep{labbe2020cosypose}, our method consists of three components (1) object detection, (2) coarse pose estimation and (3) pose refinement. 
Compared to these works, our proposed method enables generalization to novel objects not seen during training which. This requires novel approaches for the coarse model, the refiner and the training data. Our same general approach can be adapted to handle both RGB and RGB-D inputs, depending on the input modalities that are available. When depth is available we simply concatenate the depth channel to the RGB image before passing it into the network. We discuss each component in more detail below. 



\paragraph{Object Detection.}
The first step is to detect the object of interest in an RGB image.%
This is an interesting problem that has been addressed in prior work \citep{osokin2020os2d} \lucas{Add more references here} but lies outside the scope of this paper. Hence for our experiments we assume access to an object detector, but we emphasize that our pose estimation pipeline can leverage any object detector. For the BOP challenge experiments we use a MaskRCNN detector that was trained on synthetic data of the target objects. Alternatively we could leverage one-shot object detection methods such as those in OS2D \citep{osokin2020os2d} or OSOP \citep{shugurov2022cvpr:osop}. 



\begin{figure}[t]
  \centering
  \includegraphics[width=1.0\columnwidth]{figures/method.pdf}
  \caption{$\oplus$ denotes concatenation. \textbf{(a) Coarse Estimator:} Given a cropped input image the coarse module renders the object in multiple input poses $\{\tT_{\textit{CO}}^j\}$. The coarse network then classifies which rendered image best matches the observed image. \textbf{(b) Refiner:} Given an initial pose estimate $\TCO^k$ the refiner renders the objects at the estimated pose $\tT_{\textit{CO},1} \coloneq \TCO^k$ along with 3 additional viewpoints $\{\tT_{\textit{CO},i}\}_{i=2}^4$ such that the camera z-axis intersects the anchor point $\mathcal{O}$. The refiner network consumes the concatenation of the observed and rendered images and predicts an updated pose estimate $\TCO^{k+1}$.}
  \label{fig:method}
\end{figure}


\subsection{Technical Approach}


\textbf{Coarse Pose Estimation.}
Given an object detection, the goal of the coarse pose estimator is to provide an initial pose estimate $\tT_{\textit{CO}, \text{coarse}}$ which is sufficiently accurate that it can then be further improved by the refiner. This task is challenging in the case of a novel object, since the coarse estimator has no prior knowledge of the object. The input to the coarse estimator is a cropped image around the object of interest, denoted as $I_o$. An example is shown in the top of Figure \ref{fig:method} (a).

In prior work \citep{labbe2020cosypose} the coarse-estimator is a network that is trained to regress the object pose given the observed image $I_o$ and a rendered image $I_r(\tT_{\textit{CO}, \text{canonical}})$\footnote{$I_r(\TCO)$ denotes a rendered image of an object at pose $\TCO$ in camera frame} of the object in a canonical pose. However, since CosyPose \citep{labbe2020cosypose} renders only a single-view of the object it relies on prior knowledge of the object in order to recover from large pose errors, such as a 180 degree rotation. In order to generalize to novel objects our method cannot rely on object specific knowledge. Hence we propose a novel classification based approach that compares observed and rendered images of the object in a variety of poses and selects the rendered image that best matches the observed image. 
Figure \ref{fig:method} (a) gives an overview of the coarse model. At inference time the network consumes the observed image $I_o$ along with rendered images $\{I_r(\tT_{\textit{CO}}^j)\}_{j=1}^M$ of the object in a many different poses $\{\tT_{\textit{CO}}^j\}_{k=1}^M$.
For each pose $\tT_{\textit{CO}}^{j}$ the model outputs a score $\coarse(I_o, I_r(\tT_{\textit{CO}}^j)) = \xi_j$ that classifies whether pose $\tT_{\textit{CO}}^j$
is within the basin of attraction of the refiner. The highest scoring pose
$\tT_{\textit{CO}}^{j^*}, j*=\arg \max_j \xi_j$ is used as the initial pose for the refinement step.

\textbf{Pose Refinement Model.}
Given an input image and a coarse initial pose estimate $\tT_{\textit{CO}, \text{coarse}}$ the goal of the refiner is to iteratively refine the pose estimate to produce an improved estimate. The network compares the input and rendered image(s) (at the current pose estimate) and predicts a pose update. This updated pose can then be fed back to the network for further refinement.

Similar to \citep{li2018deepim, labbe2020cosypose} we train a refiner that takes as input observed $I_o$ and rendered images $I_r(\tT_{\textit{CO}}^k)$
and predicts an updated pose estimate $\TCO^{k+1} = \TCO^k \circ \Delta \tT$, whereas $  \Delta \tT \coloneqq \refiner(I_o, I_r(\TCO^k))$, see Figure \ref{fig:method} (b). Here $k$ refers to the $k^{th}$ iteration of the refiner since the refiner is able to be applied iteratively.

Our pose update uses the same parameterization as CosyPose \citep{labbe2020cosypose} which disentangles rotation and translation prediction. 
Crucially this pose update $\Delta \tT$ depends on the choice of \textit{anchor point} $\mc{O}$, see Appendix for more details \lucas{Add proof in appendix}. 
In DeepIM \citep{li2018deepim} and Cosypose \citep{labbe2020cosypose} the anchor point is chosen to be the location of a manually defined reference frame attached to the object, typically near the object centroid. 
Because the network is trained and tested on the same objects, the refiner can effectively memorize the location of this anchor point $\mc{O}_j$ for each object $j$.

For our method to generalize to novel objects, we need to inform the network about the location of the anchor point $\mc{O}$. %
The image $I_r(\tT_{\textit{CO}}^k)$
is always rendered with an image crop such that the anchor point $\mc{O}$ projects to the center of the rendered image $I_r$,
providing two pieces of information about $\mc{O}$. However there is one remaining degree of freedom: any anchor point $\mc{O}'$ that lies on the ray connecting the origin of frame $\tT_{\textit{CO}}^k$ and $\mc{O}$ would result in the same rendered image. 

We solve this problem by providing as input multiple rendered images of the object from different viewpoints. Given a pose $\tT_\textit{CO}$, we can define additional views $\{\tT_{\textit{CO}, i} \}_{i=1}^N$, where $\tT_{\textit{CO},1}$ is the standard view as in CosyPose and $\{\tT_{\textit{CO}, i} \}_{i=2}^N$ are additional views. Each rendered image $I_r(\tT_{\textit{CO},i})$ has the property that the anchor point $\mathcal{O}$ projects to the center of the image, which provides sufficient information for the network to infer the location of the anchor point via ray intersections; see Figure \ref{fig:method}(b) and the Appendix for more details. Our preferred method uses $4$ views, the standard viewpoint that matches the observed view, shown in red as $\tT_1$ in Figure \ref{fig:method}(b), and 3 additional views shown in blue. Section \ref{sec:experiments} empirically demonstrates the importance of providing multiple views to the refiner.

In addition to color images, we can also render depth and surface normal maps to further inform the network of the geometry of the novel object.  We pass these to the network by concatenating the various channels with the input. If depth images are available as part of the input observations, these can also be passed into the network by stacking the color and depth channels. We normalize both the observed and scaled depth images using the currently estimated pose $\TCO^k$ so that the network can be scale-invariant at inference time, see Appendix for more details.


\textbf{Network Architecture.} Both the coarse and refiner networks consists of a ResNet-34 backbone followed by spatial average pooling. The coarse model has a single fully-connected layer that consumes the backbone feature and outputs a classification logit. The refiner network has a single fully-connected layer that consumes the backbone feature and outputs 9 values corresponding to the pose update.









\subsection{Training Procedure}

\textbf{Training Data.}
For both the coarse and refiner models the training data consists of RGB(D)\footnote{Our method can consume either RGB or RGB-D images depending on the input modalities that are available.} images of objects with ground-truth 6D pose annotations, along with 3D models of the objects for these objects. In order for our approach to generalize to novel-objects we require a large dataset made up of diverse objects. All of of our methods are trained purely on synthetic data generated using BlenderProc \citep{denninger2019blenderproc}. We generate a dataset of 2 million images using a combination of ShapeNet \citep{shapenet2015} (abbreviated as SN) and Google-Scanned-Objects (abbreviated as GSO) \citep{downs2022google}. Similar to the BOP \citep{Hodan_undated-sl} synthetic data, we randomly sampled objects from our dataset and and dropped on a plane using a physics simulator. Materials, background textures, lighting and camera positions were randomized and images were rendered using the Blender. Example images can be seen in Figure \ref{fig:teaser}(a) and in the Appendix. Some of our ablations also use the synthetic training datasets provided by the BOP challenge \citep{Hodan_undated-sl}.

\textbf{Coarse Model.} Given an input image $I_o$ of an object $\mathcal{M}$ and a pose $\TCO$ the coarse model is trained to classify whether pose $\TCO$ is within the basin of attraction of the refiner. In other words, if the refiner were started with the initial pose estimate $\TCO^0 = \TCO'$ would it be able to estimate the ground-truth pose via iterative refinement. Given a ground-truth pose-annotation $\TCO^*$ we randomly sample poses $\TCO'$ by adding random translation and rotation to $\TCO^*$. A pose $\TCO'$ is labeled as positive if $\TCO'$ is within a threshold (5cm of translation and 15 degrees in rotation)\lucas{Check that this is accurate}\arsalan{isn't it 15 degrees standard deviation?} of the ground-truth pose $\TCO^*$ and is labeled as a negative otherwise. The model is then trained with binary cross entropy loss. 

\textbf{Refiner Model.} The refiner model is trained similarly to \citep{labbe2020cosypose}. Given an image with an object $\mathcal{M}$ at ground-truth pose $\TCO^*$ we generate a perturbed pose $\TCO'$ by applying a random translation and rotation to $\TCO^*$. Translation is sampled from a normal distribution with a standard deviations of $(0.02, 0.02, 0.05)$ centimeters and rotation is sampled as random Euler angles with a standard deviation of $15$ degrees in each axis. The network is trained to predict the relative transformation between the initial and target pose. Following \citep{labbe2020cosypose, li2018deepim} we use a symmetric disentangled loss that disentangles the prediction of depth, $x-y$ translation, and rotation. See Appendix for more details.
}


{
\section{experiments}
\color{red}
\yann{Emphasize variety of conditions in BOP challenge which makes it suited for evaluating if a method is practical for robotic applications. Different sensors, different camera parameters, etc. Prior work use different detectors, and are not available. We thus compare with other refiner methods that have only been tested on simple dataset displaying a single object on dark background.}

\label{sec:experiments}
In order to evaluate our method we run experiments on all the BOP datasets in addition to a synthetic ModelNet benchmark. Our goals are threefold: (1) Understand how our approach compares to other novel-object pose estimation methods, (2) Evaluate the performance of our refiner as compared to fully-supervised approaches like \citep{labbe2020cosypose}, and (3) Understand the effect of training-data and design-choices on performance.

\textbf{Training Data:} In order for our approach to generalize to novel-objects we require a large dataset made up of diverse objects. All of of our methods are trained purely on synthetic data generated using BlenderProc \citep{denninger2019blenderproc}. We generate a dataset of 2 million images using a combination of ShapeNet \citep{shapenet2015} (abbreviated as SN) and Google-Scanned-Objects (abbreviated as GSO) \citep{downs2022google}. Similar to the BOP \citep{Hodan_undated-sl} synthetic data, we randomly sampled objects from our dataset and and dropped on a plane using a physics simulator. Materials, background textures, lighting and camera positions were randomized and images were rendered using the Blender. Example images can be seen in Figure \ref{fig:teaser}(a) and in the Appendix. Some of our ablations use the synthetic datasets provided by the BOP challenge \citep{Hodan_undated-sl}.



\textbf{Naming convention:} Our methods are named using the following convention  \textit{(training-data)-(input-modality)-(num-views)-(rendered outputs)}. For example \textit{SN+GSO-rgbd-4-nd} is a method trained on SN and GSO objects that consumes RGB-D input and renders 4 views each with rgb, normals and depth. \textit{ycbv-rgb-1} is a method trained on YCBV PBR data, consumes RGB input and a single rendered rgb image, which corresponds to the setting of CosyPose \citep{labbe2020cosypose}. Our preferred configurations are \textit{Ours (RGB) = SN+GSO-rgb-4-n} and \textit{Ours (RGB-D) = SN+GSO-rgbd-4-nd}.


\subsection{6D pose estimation of novel objects.}

Table \ref{tab:bop} reports results of our novel-object pose estimation method on the datasets from the BOP challenge \citep{Hodan_undated-sl}. Note that since novel instance detection is outside the scope of this paper we use the Mask-RCNN network trained on the BOP PBR datasets for object detection. The bottom section of the table compares our performance with Drost \citep{}, OSOP \cite{shugurov2022cvpr:osop}, and Zephyr \citep{okorn2021icra:zephyr}. An apples-to-apples comparison is challenging since we use an object detector trained on the target objects \lucas{We need a better justification here}. However, across all datasets for which they report results (LM-O, HB, YCB-V) our approach outperforms all baselines while being trained purely on synthetic data. Adding depth input to our approach significantly boosts performance by helping to resolve the z-translation component of $\TCO$. Additionally, since our approach uses a pose-refiner our method can be used to refine arbitrary initial pose estimates. In particular our method could be used to refine the initial estimates from \citep{shugurov2022cvpr:osop,okorn2021icra:zephyr}.


Table \ref{tab:results-modelnet} illustrates the performance of the refiner on the ModelNet benchmark from \citep{li2018deepim}. This dataset consists of renderings of isolated ModelNet \citep{wu20153d} objects on a black background. The network is then provided an initial pose that is a perturbation of the ground-truth pose using the parameters from DeepIM \citep{li2018deepim}\footnote{The pose perturbation is sampled from a normal distribution with standard deviation of $(0.01, 0.01, 0.05)$ in translation and $15$ degrees for each of roll, pitch and yaw}. \textit{Ours (RGB)} outperforms DeepIM \citep{li2018deepim}, Multi-AAE \citep{Sundermeyer_2020_CVPR} and LatentFusion \citep{park2020cvpr:latentfusion} across all metrics. \textit{Ours (RGB-D)} performs slightly worse than \textit{Ours (RGB)} but generally still better than the baselines. We hypothesize that this drop in performance from RGB to RGB-D on the ModelNet benchmark is due to the domain gap between the depth images from the ModelNet benchmark and those in our training data.

\subsection{Novel-Object Refiner vs. Supervised Refiner}
In this section we aim to understand if novel-object refiners\footnote{A novel-object is defined as an object that has not been seen at training time} can achieve competitive performance with refiners that are trained on the test objects. To investigate this we again consider the BOP challenge \citep{Hodan_undated-sl} datasets. In order to enable a fair comparison all methods use the same coarse refiner from CosyPose \citep{labbe2020cosypose} (which has been trained on synthetic data of the test objects). As shown in the middle rows of Table \ref{tab:bop} \textit{Ours (RGB)} matches or outperforms the \textit{CosyPose} refiner on all BOP datasets even though it has never seen the test objects during training. As before, adding depth significantly improves performance as shown in \textit{Ours (RGB-D)}. The methods \textit{Ours (RGB) = SN+GSO-rgb-4-n} and \textit{BOP-rgb-4-n} differ only in the training data with \textit{BOP-rgb-4-n} being trained on the test objects. Interestingly \textit{Ours (RGB)} achieves comparable or better performance across all BOP datasets, showing that novel-object refiners can be competitive with refiners trained on the test objects. A similar trend is performance is seen for models that consume depth input by comparing \textit{Ours (RGB-D)} and \textit{BOP-rgbd-4-nd}. Again, our \textit{Ours (RGB-D)} performs on-par or better than a model trained on the test objects.

\subsection{Ablations}
In this section we perform ablations of our approach to validate our main contributions.

\textbf{Number of views:} As discussed in Section \ref{subsec:pose_refinement} in order to generate to novel objects the refiner must have information about the anchor point $\mc{O}$. In our method we accomplish this by using 4 rendered views. Table \ref{tab:ablation} (a) shows that the performance of the refiner steadily increases as we increase the number of views from $1$ to $4$, validating our design choice. Multiple views may also help the network to understand what the object looks like from alternate viewpoints, thus potentially helping the refiner to overcome large initial pose errors.

\textbf{Data Augmentation:} Depth images from consumer grade depth sensors are often noisy and incomplete. Since our method is trained solely on synthetic data, where depth images are perfect, there exists a significant domain gap. To illustrate this we trained a variant of our method \textit{Ours (RGB-D) light-aug} that uses relatively \textit{light} data augmentation on the depth images during training, see Appendix for details. The results in in Table \ref{tab:ablation} \lucas{Add results} demonstrate that heavy data augmentation on the depth images, as in \textit{Ours (RGB-D)} is critical to ensuring good sim-to-real transfer. In fact since we during training of \textit{Ours (RGB-D)} we sometimes set the depth images to zero, \textit{Ours (RGB-D)} is actually able to properly refine pose estimates when input depth images are set to zero,  with performance similar to \textit{Ours (RGB)}, thus demonstrating the robustness of the model. \lucas{This is anecdotal, but seems to work. Do we need more justification?}



\subsection{Importance of the training data}
\yann{These results suggest show we could improve performance with more high-quality 3D models. Thanks to the fully learned nature of our method. Show importance of training data. We will make our dataset publicate and hope it will stimulate the development of methods, including for detection for which the data can be used to train zero-shot detection methods.}
\yann{Models are trained for half the time due to the resources required for training one model.}

Table \ref{tab:ablation} (a) shows the effect of using different sets of training objects on performance. The table shows that a diverse set of objects (GSO + ShapeNet) works best and that just using ShapeNet objects hurts performance. We hypothesize that this is most likely due to a domain gap between the ShapeNet objects, which are mostly textureless, and some of the BOP datasets (e.g. YCBV) that contain highly textured objects, see Appendix for a complete set of results broken out by dataset.

\textbf{Number of training objects and images:} As can be seen in table \ref{tab:ablation} (b) performance increase as you increase both the number of training images and also the number of distinct objects demonstrating that a large and diverse dataset is critical for good performance.

\subsection{Real-world experiments.}
\lucas{Do some robot grasping experiments time-permitting.}



\arsalan{Do we have results with gt classifier and different number of views. to see how much performance we lose by just using classification. This is to highlight whether sampling init point is the most significant bit or improving the classification}
}

\subsection{Limitations}
While MegaPose shows promising results in robot experiments and 6D pose estimation benchmarks, there is still room for improvement. The most common failure mode is due to inaccurate initial pose estimates from the coarse model. The refiner model is trained to correct the poses if the relative pose error is within a constrained range, but can fail if the initial error is too large. The success of the MegaPose pipeline depends on whether any of the coarse pose hypotheses $\{ \tT_{\textit{CO}}^j \}_{j=1}^M$ are within the basin of attraction of the refiner model. There are multiple potential approaches to alleviate this problem. We can increase the number of sampled initial poses $M$ at the expense of increased inference time, improve the accuracy of the coarse model, and increase the basin of attraction for refinement model.


{
\section{Related work.}
\color{red}
\paragraph{6D pose estimation of rigid objects.} This computer vision problem~\cite{Roberts1963-ck,Lowe1987-yf,Lowe1999-bf} was originally solved by estimating the
pose from 2D-3D correspondences obtained via local invariant features~\cite{Lowe1999-bf,bay2006surf,Collet2010-zj,Collet2011-lj}, or by
template-matching~\cite{Hinterstoisser2011-es} using RGB images. Both these strategies have been
revisited using convolutional neural networks (CNNs). A set of sparse \cite{Rad2017-de,Tremblay2018-deep,Kehl2017-ssd,Tekin2017-hp,peng2019pvnet,pavlakos20176,hu2019segmentation} or dense \cite{Xiang2018-dv,Park2019-od,song2020hybridpose,zakharov2019dpod,haugaard2021surfemb} features is detected on the object in the image using a CNN and the resulting 2D-to-3D correspondences are used to recover
the camera pose using PnP~\cite{lepetit2009epnp}. The best performing
methods for 6D pose estimation from RGB images are now based on variants of the {\em \rendercomp} strategy \cite{oberweger2015training,Rad2017-de,li2018deepim,manhardt2018deep,oberweger2019generalized,labbe2020cosypose,zakharov2019dpod,di2021iccv:sopose} and are approaching the accuracy of methods using depth as input~\cite{hodan2020bop,Hodan_undated-sl,li2018deepim,labbe2020cosypose} \lucas{It shouldn'be be presented as RGB vs. RGBD. Of course you should use depth when you have it, but it is also a selling point of our approach that it doesn't require depth}.
\cite{Di_2021_SO_Pose}

\paragraph{6D pose estimation of novel objects without CAD models.} Category-level 6D pose estimation. Assumes similarities between training cateogries. CAtegory is not simple. For example
Rely on category-level information~\cite{wang20206,manuelli2019kpam}. But its not easy to define what a category is and where are its limits for any objects such as industrial ones. Some others address a similar to ours where information on the object is available in the form of a set of reference views~\cite{liu2022arxiv:gen6d}


\paragraph{6D pose estimation of novel objects with CAD models.}

RGB-D methods~\cite{drost2010model,densefusion,6pack,}

\yann{Be careful about not forgetting depth-based methods. This paragraph was almost copied from cosypose-PAMI where RGB-only was the focus.}


\paragraph{One Shot 6D Object Pose Estimation}
The methods that have

One shot object pose estimation methods rely on comparing some reference views of the object with the current view of the object in query image. One line of work takes the brute force approach and samples a dense set of hypothesis and score the hypothesis by comparing the query image and reference of views of the object rendered at the hypothesized poses~\cite{park2020cvpr:latentfusion, okorn2021icra:zephyr, Sundermeyer_2020_CVPR}. The reference views are generated either from registered views of the object~\cite{sun2022cvpr:onepose,park2020cvpr:latentfusion} or from textured CAD models~\cite{li2018deepim, Sundermeyer_2020_CVPR, liu2022arxiv:gen6d, shugurov2022cvpr:osop}. To compare the reference view and query image, \cite{Sundermeyer_2020_CVPR, nguyen2022cvpr:templatepose} use embeddings that capture the appearance of objects. LatentFusion~\cite{park2020cvpr:latentfusion} uses the pixelwise L2 distance between the rendering of object and query image to guide the sampling. Both of these approaches are sensitive to occlusions. On the other hand, \cite{labbe2020cosypose, li2018deepim} use a refiner model that directly predicts a relative transform between the query image and reference view, resulting in better robustness to occlusions. OSOP~\cite{shugurov2022cvpr:osop} make the relative transformation prediction more explicit by predicting 2D-2D correspondences between an observed and rendered image, and solve for pose using PnP or Kabsch, making the inferece slower compared to directly predicting refinement transform. To mitigate the sampling complexity at the inference time, a coarse model is used to find the closest reference view to the query object~\cite{sun2022cvpr:onepose, liu2022arxiv:gen6d}.  






\yann{LF uses object masks and L2 objective}
\yann{Don't forget about~\cite{xiao2021-3dv:posecontrast}}
\yann{paragraph with~\cite{wohlhart2015learning,balntas2017pose,nguyen2022cvpr:templatepose}.}
\yann{Our coarse estimator draws similarities with hypothesis scoring methods. These methods have used voting~\cite{} or more recently learned~\cite{okorn2021icra:zephyr}}
\yann{Paragraph with "Traditional non learning-based methods" such as PPF before talking about learning based methods~\cite{drost2010model,vidal2018method}}.
\yann{Can have a paragraph about category level pose estimation but these methods}
\yann{Talk about LF, (also refered to as zero-shot poes esimation methods)~\cite{park2020cvpr:latentfusion,Sundermeyer_2020_CVPR,nguyen2022cvpr:templatepose,xiao2019bmvc:posefromshape}}
\yann{paragraph on self-supervised methods~\cite{wang2020self6d,Wang_2021_self6dpp}}
\yann{Say something about training data and limitations. In contrast, we don't need to deal with any training data once the model is trained on our large scale dataset. Zephyr, OSOP train only a few hundreds objects and demonstrate limited generlaization. Gen6D trains on thousands of objects, but single object and no results on occluded scenes. BTW this paper will get in at ECCV.}
\yann{Synthetic data~\cite{tobin2017domain,Tremblay2018-deep}}
\yann{paragraph on methods that do not require CAD models such as~\cite{yen2021inerf,sun2022cvpr:onepose}}

ZePHyR~\cite{okorn2021icra:zephyr}.
DeepIM~\cite{li2018deepim}.
LatentFusion~\cite{park2020cvpr:latentfusion}. At test time, it requires (i) depth, (ii) mask of the object, (ii) multiple real images of the new object with annotated relative camera poses. Refined pose
MP-Encoder~\cite{Sundermeyer_2020_CVPR}, AAE~\cite{sundermeyer2018implicit}. Orientation estimation is done by matching the descriptors of the query with multiple synthetic views of the 3D model. It relies on auto-encoder, the alignment is only coarse and requires XX to refine object pose.

Gen6D~\cite{liu2022arxiv:gen6d}.

TemplatePose~\cite{nguyen2022cvpr:templatepose}.
PoseContrast~\cite{} (extract features in a single image, not robust to occlusions, good argument from Gen6D.)
OSOP~\cite{shugurov2022cvpr:osop}.

OnePose~\cite{sun2022cvpr:onepose}

FS6D~\cite{he2022cvpr:fs6d}

Coupled iterative refinement~\cite{lipson2022cvpr:coupitref}

Optimal pose~\cite{shi2021rss:optimalpose}.  It seems to be category-level estimation.

CenterPose~\cite{lin2022icra:centerpose}. 

Masked autoencoders~\cite{he2021arxiv:maskedae}

PoseContrast~\cite{xiao2021-3dv:posecontrast}. 

Self6D~\cite{wang2020self6d}: introduced a self-supervised learning pipeline, leveraging a differentiable renderer, to refine a synthetically trained pose predictor on unlabeled real images. (Orthogonal to our work)
}
